Resource-Bound Quantification for Graph Transformation

Graph transformation has been used to model concurrent systems in software engineering, as well as in biochemistry and life sciences. The application of a transformation rule can be characterised algebraically as construction of a double-pushout (DPO) diagram in the category of graphs. We show how intuitionistic linear logic can be extended with resource-bound quantification, allowing for an implicit handling of the DPO conditions, and how resource logic can be used to reason about graph transformation systems.

==> eptcsdata.tex <==
\providecommand{\event}{M. Florido and I. Mackie (Eds.): First International\\
Workshop on Linearity (LINEARITY 2009)}
\providecommand{\volume}{22}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{14}
\providecommand{\eid}{2}

